Can a Single Model Master Both Multi-turn Conversations and Tool Use? CoALM: A Unified Conversational Agentic Language Model

Large Language Models (LLMs) with API-calling capabilities enabled building effective Language Agents (LA), while also revolutionizing the conventional task-oriented dialogue (TOD) paradigm. However, current approaches face a critical dilemma: TOD systems are often trained on a limited set of target APIs, requiring new data to maintain their quality when interfacing with new services, while LAs are not trained to maintain user intent over multi-turn conversations. Because both robust multi-turn management and advanced function calling are crucial for effective conversational agents, we evaluate these skills on three popular benchmarks: MultiWOZ 2.4 (TOD), BFCL V3 (LA), and API-Bank (LA), and our analyses reveal that specialized approaches excel in one domain but underperform in the other. To bridge this chasm, we introduce CoALM (Conversational Agentic Language Model), a unified approach that integrates both conversational and agentic capabilities. We created CoALM-IT, a carefully constructed multi-task dataset that interleave multi-turn ReAct reasoning with complex API usage. Using CoALM-IT, we train three models CoALM 8B, CoALM 70B, and CoALM 405B, which outperform top domain-specific models, including GPT-4o, across all three benchmarks. This demonstrates the feasibility of a single model approach for both TOD and LA, setting a new standard for conversational agents.

==> prompts/attraction-data-sample.tex <==
\begin{table*}
\scriptsize
Output dialogue sample for attraction domain, generated by GPT4o-mini.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
System:  \\
User: can you please help me find a place to go ? \\
System: i have found 79 place -s for you to go . do you have any specific ideas in mind ? \\
User: i would like a sports place in the centre please . \\
System: there are no results matching your query . can i try a different area or type ? \\
User: okay , are there any cinemas in the centre ? \\
System: we have vue cinema \\
User: okay that will work . can you please tell me their phone number , postcode and the entrance fee ? \\
System: vue can be reached at 08712240240 , the postcode is cb11ps . i do not have entrance fee information , i am sorry . \\
User: no worries , i'll give them a call and find out . thanks so much for all your help , goodbye . \\
 \\
 \\
 \\
User: Can you please help me find a place to go? \\
System: I have found 79 places for you to go. Do you have any specific ideas in mind? \\
 \\
User: I would like a sports place in the centre, please. \\
Thought: I need to call an API to find attractions that fit the criteria. \\
API Name: [Attraction: quer\_attractions] \\
API Input: {"type": "multiple sports", "area": "centre"} \\
API Result: [] \\
Thought: There are no results matching the given criteria. I should ask the user if they want to try a different area or type. \\
Response: There are no results matching your query. Can I try a different area or type? \\
 \\
User: Okay, are there any cinemas in the centre? \\
Thought: I need to call an API to find cinemas in the centre. \\
API Name: [Attraction: query\_attractions] \\
API Input: {"type": "cinema", "area": "centre"}
API Result: [{"address": "cambridge leisure park, clifton way", "area": "south", "entrance fee": "?", "id": "21", "location": [52.1901222222222, 0.136991666666667], "name": "cineworld cinema", "openhours": "?", "phone": "00872208000", "postcode": "cb17dy", "pricerange": "?", "type": "cinema"}, {"address": "the grafton centre, east road", "area": "centre", "entrance fee": "?", "id": "75", "location": [52.20571, 0.131061], "name": "vue cinema", "openhours": "?", "phone": "08712240240", "postcode": "cb11ps", "pricerange": "?", "type": "cinema"}] \\
Thought: There is a cinema in the centre that matches the user's criteria. \\
Response: We have Vue Cinema. \\
 \\
User: Okay, that will work. Can you please tell me their phone number, postcode, and the entrance fee? \\
Thought: I need to provide the user with the requested information about Vue Cinema. \\
Response: Vue Cinema can be reached at 08712240240, the postcode is CB11PS. I do not have entrance fee information, I am sorry. \\
 \\
User: No worries, I'll give them a call and find out. Thanks so much for all your help, goodbye. \\
Thought: The user is satisfied with the information provided and will call the cinema for further details. \\
Response: You're welcome! Have a great day, goodbye! \\
 \\
\bottomrule \\
\end{tabular}
\end{table*}

==> prompts/hotel-data-sample.tex <==
\begin{table*}
\scriptsize
Output dialogue sample for hotel domain, generated by GPT4o-mini.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
System: \\
User: am looking for a place to to stay that has cheap price range it should be in a type of hotel\\
System: okay , do you have a specific area you want to stay in ?\\
User: no , i just need to make sure it s cheap . oh , and i need parking\\
System: i found 1 cheap hotel for you that include -s parking . do you like me to book it ?\\
User: yes , please . 6 people 3 nights starting on tuesday .\\
System: i am sorry but i was not able to book that for you for tuesday . is there another day you would like to stay or perhaps a shorter stay ?\\
User: how about only 2 nights .\\
System: booking was successful . reference number is : 7gawk763 . anything else i can do for you ?\\
User: no , that will be all . goodbye .\\
 \\
 \\
 \\
User: am looking for a place to stay that has cheap price range it should be in a type of hotel  \\
System: okay , do you have a specific area you want to stay in ?  \\
Thought: I need to call an API to find hotels that match the user's criteria for price range and type.  \\
API Name: Hotel: query\_hotels  \\
API Input: {"pricerange": "cheap", "type": "hotel"}  \\
API Result: [{"address": "56 saint barnabas road", "area": "centre", "internet": "yes", "parking": "yes", "id": "2", "location": [52.1986444444444, 0.138133333333333], "name": "alexander bed and breakfast", "phone": "01223525725", "postcode": "cb12de", "price": {"double": "50", "single": "40"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "517a coldham lane", "area": "east", "internet": "yes", "parking": "yes", "id": "3", "location": [52.1963733, 0.1987426], "name": "allenbell", "phone": "01223210353", "postcode": "cb13js", "price": {"double": "60", "family": "90", "single": "35"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "710 newmarket road", "area": "east", "internet": "yes", "parking": "yes", "id": "8", "location": [52.2176534, 0.1747439], "name": "autumn house", "phone": "01223575122", "postcode": "cb58rs", "price": {"double": "60", "family": "90", "single": "40"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "328a histon road", "area": "north", "internet": "yes", "parking": "yes", "id": "13", "location": [52.227589, 0.112288], "name": "city centre north b and b", "phone": "01223312843", "postcode": "cb43ht", "price": {"single": "40"}, "pricerange": "cheap", "stars": "0", "takesbookings": "yes", "type": "hotel"}, {"address": "41 warkworth street", "area": "centre", "internet": "yes", "parking": "yes", "id": "15", "location": [52.20439812598512, 0.13059139251708984], "name": "el shaddai", "phone": "01223327978", "postcode": "cb11eg", "price": {"double": "60", "family": "62", "single": "40"}, "pricerange": "cheap", "stars": "0", "takesbookings": "yes", "type": "hotel"}, {"address": "144 thornton road", "area": "west", "internet": "yes", "parking": "yes", "id": "17", "location": [52.226235, 0.091796], "name": "finches bed and breakfast", "phone": "01223276653", "postcode": "cb30nd", "price": {"double": "50", "single": "50"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "732-734 newmarket road", "area": "east", "internet": "yes", "parking": "yes", "id": "24", "location": [52.2176534, 0.1747439], "name": "leverton house", "phone": "01223292094", "postcode": "cb58rs", "price": {"double": "60", "family": "90", "single": "40"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "53 roseford road", "area": "south", "internet": "yes", "parking": "yes", "id": "27", "location": [52.1725982, 0.1112224], "name": "rosa's bed and breakfast", "phone": "01223512596", "postcode": "cb22ha", "price": {"single": "25"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "back lane, cambourne", "area": "west", "internet": "yes", "parking": "yes", "id": "28", "location": [52.2213805555556, -0.0680333333333333], "name": "the cambridge belfry", "phone": "01954714600", "postcode": "cb236bw", "price": {"double": "60", "single": "60"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}, {"address": "152 chesterton road", "area": "north", "internet": "yes", "parking": "yes", "id": "32", "location": [52.2309912, 0.1295545], "name": "worth house", "phone": "01223316074", "postcode": "cb41da", "price": {"double": "60", "family": "85", "single": "49"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}] \\ 
Thought: The results contain too many hotels. I need to ask the user for more constraints.  \\
\\
User: no , i just need to make sure it s cheap . oh , and i need parking  \\
System: i found 1 cheap hotel for you that include -s parking . do you like me to book it ?  \\
Thought: I need to call an API to check if this hotel can be booked.  \\
API Name: Hotel: query\_hotels  \\
API Input: {"pricerange": "cheap", "type": "hotel", "parking": "yes"}  \\
API Result: [{"address": "56 saint barnabas road", "area": "centre", "internet": "yes", "parking": "yes", "id": "2", "location": [52.1986444444444, 0.138133333333333], "name": "alexander bed and breakfast", "phone": "01223525725", "postcode": "cb12de", "price": {"double": "50", "single": "40"}, "pricerange": "cheap", "stars": "4", "takesbookings": "yes", "type": "hotel"}]  \\
Thought: The hotel found matches the user's criteria and is available for booking.  \\
\\
User: yes , please . 6 people 3 nights starting on tuesday .  \\
System: i am sorry but i was not able to book that for you for tuesday . is there another day you would like to stay or perhaps a shorter stay ?  \\
Thought: I need to attempt to book the hotel for the user, but if it fails, I should offer a shorter stay.  \\
API Name: Hotel: book\_hotel  \\
API Input: {"hotel\_id": "2", "people": 6, "nights": 3, "start\_day": "tuesday"}  \\
API Result: {"success": false}  \\
Thought: The booking failed. I will ask the user if they would like to reduce the number of nights.  \\
\\
User: how about only 2 nights .  \\
System: booking was successful . reference number is : 7gawk763 . anything else i can do for you ?  \\
Thought: I need to confirm that the booking was successful and provide the reference number to the user.  \\
API Name: Hotel: book\_hotel  \\
API Input: {"hotel\_id": "2", "people": 6, "nights": 2, "start\_day": "tuesday"}  \\
API Result: {"success": true, "reference\_number": "7gawk763"}  \\
Thought: The booking was successful and I have provided the reference number to the user.  \\
\\
User: no , that will be all . goodbye .  \\
System: Thought: I don't need an API and want to respond to the user.  \\
Response: Goodbye! Have a great day!\\
\bottomrule
\end{tabular}
\end{table*}

==> prompts/react-data-generation-prompts/kvret-data-generation-prompt.tex <==
\begin{table*}
\scriptsize
API-driven conversation prompt for KVRET.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
\# Role Description: \\
You are an advanced AI assistant specializing in conversational dialogues, specifically in the travel domain. You can act both as a system (providing services) and a user (interacting with the system) to assist users in completing complex tasks.  \\
Each task may involve multiple sub-tasks, such as finding restaurants, making reservations, booking hotels, and locating attractions. \\
 \\
\# Task Information: \\
- You are asked to create multi-turn dialogues between a user and a system, based on provided Input Dialogue Items. \\
- The dialogues should be converted to follow a specific Output Format, which includes reasoning on whether an API call is needed, or, if the system can respond directly. The generated dataset should be in the format as: User - Thought\_User - API - API Input Arguments - API Result - Thought\_API - System, or, User - Thought\_User - System. For each user utterance, the system must determine whether to call an API by reasoning through the context provided in "Thought\_User:". \\
- If the system decides that an API call is necessary, include "API Name:", "API Input:", and "API Result", followed by a "Thought\_API:" for API reasoning. Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- If the system determines that an API call is not necessary, directly respond to the user, including "Thought\_User:" as reasoning and the provide response to the user as "System:". \\
 \\
\# Available Functions: \\
1. schedule(agenda, day, time, event, party, room) \\
2. weather(location, day, weather\_attribute) \\
3. navigate(distance, address, point\_of\_interest, type, traffic\_information) \\
 \\
\# Output Format: \\
- If an API Call is Needed: \\
\quad	User: [User Input] \\
\quad    Thought\_User: I need to call an API. \\
\quad    API Name: [Available APIs: schedule(agenda, day, time, event, party, room), weather(location, day, weather\_attribute), navigate(distance, address, point\_of\_interest, type, traffic\_information)] \\
\quad    API Input: [The input parameters for the API function] \\
 \quad   API Result: [API output] \\
 \quad   Thought\_API: [2nd thought after API Result that ensure if the information is enough before the system response] \\
\quad	System: [Your system response here] \\
 \\
- If an API Call is Not Needed: \\
\quad	User: [User Input] \\
 \quad   Thought\_User: I don't need an API and want to respond to the user. \\
 \quad   System: [Your system response here] \\
 \\
\# Objective:  \\
- Convert the reference dialogue using the provided Output Format above. Ensure that each system utterance follows logical reasoning, determining whether an API call is needed and structuring the output accordingly. \\
- If there are too many results returned by API results from database, the AI Assistant should ask the user for more constraints. \\
 \\
\# Sample Example \\
User: Add Don and Sherri to my "Meditate to Sounds of Nature" playlist.   \\
Thought\_User: The user wants to add two artists to a specific playlist. I'll need to extract the playlist name and the artists' names.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'artists': ['Don Sherri']}   \\
API Result: {'status': 'success', 'message': 'Don and Sherri have been added to your playlist.'}   \\
Thought\_API: The API call was successful, and the artists were added to the playlist. I need to inform the user about this.   \\
System: Don and Sherri have been successfully added to your "Meditate to Sounds of Nature" playlist. Enjoy your music!   \\
 \\
User: Thank you for adding them. I think I can add more songs to the playlist. \\
Thought\_User: I don't need an API call for that, I want to respond to the user.  \\
System: Would you like to add more songs?   \\
 \\
User: Yes, please add "Calm River" to the playlist.   \\
Thought\_User: The user wants to add another song to the playlist. I'll note the song title and proceed with the request.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'songs': ['Calm River']}   \\
API Result: {'status': 'success', 'message': 'Calm River has been added to your playlist.'}   \\
Thought\_API: The song was successfully added. I should let the user know.   \\
System: "Calm River" has been successfully added to your "Meditate to Sounds of Nature" playlist. Would you like to do anything else?   \\
 \\
User: No, that's all for now. Thank you!   \\
Thought\_User: The user is satisfied and doesn't need further assistance. I should acknowledge their gratitude.   \\
System: You're welcome! If you need anything else, feel free to ask. Enjoy your relaxing music! \\
 \\
\# Input Dialogue Items: \\
{"turn": 0, "user": "Find me the address of a shopping center .", "state": "[navigate] type : shopping center", "system\_response\_raw": "We 're near town and country and midtown shopping center , i suggest you the last one because is nearer and there is less traffic on the way"}
{"turn": 1, "user": "Then i will trust you car , do n't make me regret it or there will be no more gasoline for you ... please pick the shortest distance and let 's go there , thank you !", "state": "[navigate] point of interest : town and country", "system\_response\_raw": "Okay heading to midtown shopping center at 338 alester ave ."}\\ \bottomrule
\end{tabular}
\end{table*}

==> prompts/react-data-generation-prompts/msr-data-generation-prompt.tex <==
\begin{table*}
\scriptsize
API-driven conversation prompt for MSR-E2E.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
\# Role Description: \\
You are an advanced AI assistant specializing in conversational dialogues, specifically in the travel domain. You can act both as a system (providing services) and a user (interacting with the system) to assist users in completing complex tasks.  \\
Each task may involve multiple sub-tasks, such as finding restaurants, making reservations, booking hotels, and locating attractions. \\
 \\
\# Task Information: \\
- You are asked to create multi-turn dialogues between a user and a system, based on provided Input Dialogue Items. \\
- The dialogues should be converted to follow a specific Output Format, which includes reasoning on whether an API call is needed, or, if the system can respond directly. The generated dataset should be in the format as: User - Thought\_User - API - API Input Arguments - API Result - Thought\_API - System, or, User - Thought\_User - System. For each user utterance, the system must determine whether to call an API by reasoning through the context provided in "Thought\_User:". \\
- If the system decides that an API call is necessary, include "API Name:", "API Input:", and "API Result", followed by a "Thought\_API:" for API reasoning. Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- If the system determines that an API call is not necessary, directly respond to the user, including "Thought\_User:" as reasoning and the provide response to the user as "System:". \\
 \\
\# Available Functions: \\
1. request(ticket;moviename=Zoolander 2;date=tomorrow;theater=Regal Meridian 16;city=Seattle;starttime=9:25 PM;numberofpeople=2)
2. inform(taskcomplete;numberofpeople=2;moviename=Zoolander 2)
 \\
\# Output Format: \\
- If an API Call is Needed: \\
\quad	User: [User Input] \\
\quad    Thought\_User: I need to call an API. \\
\quad    API Name: [Available APIs: request(),inform(),] \\
\quad    API Input: [The input parameters for the API function] \\
 \quad   API Result: [API output] \\
 \quad   Thought\_API: [2nd thought after API Result that ensure if the information is enough before the system response] \\
\quad	System: [Your system response here] \\
 \\
- If an API Call is Not Needed: \\
\quad	User: [User Input] \\
 \quad   Thought\_User: I don't need an API and want to respond to the user. \\
 \quad   System: [Your system response here] \\
 \\
\# Objective:  \\
- Convert the reference dialogue using the provided Output Format above. Ensure that each system utterance follows logical reasoning, determining whether an API call is needed and structuring the output accordingly. \\
- If there are too many results returned by API results from database, the AI Assistant should ask the user for more constraints. \\
 \\
\# Sample Example \\
User: Add Don and Sherri to my "Meditate to Sounds of Nature" playlist.   \\
Thought\_User: The user wants to add two artists to a specific playlist. I'll need to extract the playlist name and the artists' names.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'artists': ['Don Sherri']}   \\
API Result: {'status': 'success', 'message': 'Don and Sherri have been added to your playlist.'}   \\
Thought\_API: The API call was successful, and the artists were added to the playlist. I need to inform the user about this.   \\
System: Don and Sherri have been successfully added to your "Meditate to Sounds of Nature" playlist. Enjoy your music!   \\
 \\
User: Thank you for adding them. I think I can add more songs to the playlist. \\
Thought\_User: I don't need an API call for that, I want to respond to the user.  \\
System: Would you like to add more songs?   \\
 \\
User: Yes, please add "Calm River" to the playlist.   \\
Thought\_User: The user wants to add another song to the playlist. I'll note the song title and proceed with the request.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'songs': ['Calm River']}   \\
API Result: {'status': 'success', 'message': 'Calm River has been added to your playlist.'}   \\
Thought\_API: The song was successfully added. I should let the user know.   \\
System: "Calm River" has been successfully added to your "Meditate to Sounds of Nature" playlist. Would you like to do anything else?   \\
 \\
User: No, that's all for now. Thank you!   \\
Thought\_User: The user is satisfied and doesn't need further assistance. I should acknowledge their gratitude.   \\
System: You're welcome! If you need anything else, feel free to ask. Enjoy your relaxing music! \\
 \\
\# Input Dialogue Items: \\
{'message\_from': 'user', 'message\_text': "I'd like 2 tickets to see Zoolander 2 tomorrow at Regal Meridian 16 theater in Seattle at 9:25 PM", 'dialog\_acts': [['request(ticket;moviename=Zoolander 2;date=tomorrow;theater=Regal Meridian 16;city=Seattle;starttime=9:25 PM;numberofpeople=2)']]} \\
{'message\_from': 'agent', 'message\_text': 'Okay, your purchase of 2 tickets for Zoolander 2 is confirmed.', 'dialog\_acts': [['inform(taskcomplete;numberofpeople=2;moviename=Zoolander 2)']]} \\
\bottomrule
\end{tabular}
\end{table*}

==> prompts/react-data-generation-prompts/multiwoz-data-generation-prompt-ver2.tex <==
\begin{table*}
\scriptsize
API-though-conversation data generation Prompt for MultiWOZ 2.4.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
\# Role Description: \\
You are an advanced AI assistant specializing in conversational dialogues, specifically in the travel domain. You can act both as a system (providing services) and a user (interacting with the system) to assist users in completing complex tasks. \\
Each task may involve multiple sub-tasks, such as finding restaurants, making reservations, booking hotels, and locating attractions.\\
\\
\# Task Information:\\
- You are asked to create multi-turn dialogues between a user and a system, based on provided Input Dialogue Items.\\
- The dialogues should be converted to follow a specific Output Format, which includes reasoning on whether an API call is needed, or, if the system can respond directly.\\
- The generated dataset should be in the format as: User - Thought\_User - API - API Input Arguments - API Result - Thought\_API - System, or, User - Thought\_User - System. \\
- For each user utterance, the system must determine whether to call an API by reasoning through the context provided in "Thought\_User:".\\
- If the system decides that an API call is necessary, include "API Name:", "API Input:", and "API Result", followed by a "Thought\_API:" for API reasoning. Call the right API from # Avaliable Functions and provide the necessary input arguments to fulfill the user's request. If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values.\\
- If the system determines that an API call is not necessary, directly respond to the user, including "Thought\_User:" as reasoning and the provide response to the user as "System:".\\
\\
\# Available Functions:\\
"functions": [\\
    {\\
        "name": "query\_restaurants",\\
        "description": "Finds a restaurant that matches user criteria, such as area, food type, or price range.",\\
        "parameters": {\\
            "type": "object",\\
            "properties": {\\
                "area": {\\
                    "type": "string",\\
                    "description": "The area for which to look for restaurants, such as the center of town or east.",\\
                    "enum": ["east", "west", "south", "north", "centre"]\\
                },\\
                "pricerange": {\\
                    "type": "string",\\
                    "description": "The price range of the restaurant, such as, cheap or expensive.",\\
                    "enum": ["cheap", "moderate", "expensive"]\\
                },\\
                "food": {\\
                    "type": "string",\\
                    "description": "The cuisine of the food served in the restaurant, such as Indian or Italian."\\
                }\\
            },\\
            "required": []\\
        }\\
    },\\
    {\\
     	"name": "book\_restaurant",\\
	    "description": "Makes a table reservation for the requested restaurant, day, time, and number of people.",\\
	    "parameters": {\\
            "type": "object",\\
            "properties": {\\
		        "people": {\\
                    "type": "integer",\\
                    "description": "The number of people for which to book a table, such as 2 or 4."\\
		        },\\
                "name": {\\
                    "type": "string",\\
                    "description": "The name of the restaurant to book a table at, such as Il Fornaio or Cascal.\\"
		        },\\
                "day": {\\
                    "type": "string",\\
                    "description": "The day of the restaurant reservation, such as tomorrow or Wednesday."
		        },\\
		        "time": {\\
                    "type": "string",\\
                    "description": "The time of the restaurant reservation, such as 7pm or 18:00."\\
		        }\\
            },\\
            "required": []\\
	    }\\
    },\\
    {\\
        "name": "query\_hotels",\\
        "description": "Finds a hotel that matches user criteria, such as area, number of stars, or price range.",\\
        "parameters": {\\
            "type": "object",\\
            "properties": {\\
                "area": {\\
                    "type": "string",\\
                    "description": "The area for which to look for hotels, such as the center of town or east.",\\
                    "enum": ["east", "west", "south", "north", "center"]\\
                },\\
                "pricerange": {\\
                    "type": "string",\\
                    "description": "The price range of the hotel, such as, cheap or expensive.",\\
                    "enum": ["cheap", "moderate", "expensive"]\\
                },\\
                "stars": {\\
                    "type": "integer",\\
                    "description": "The number of stars for the hotel that is sought, such as three or four."\\
                },\\
                "type": {\\
                    "type": "string",\\
                    "description": "The type of the hotel that is sought, such as hotel or guest house."\\
                },\\
                "internet": {\\
                    "type": "string",\\
                    "description": "The internet requirements for the hotel that is sought, for example, yes or no."\\
                },\\
                "parking": {\\
                    "type": "string",\\
                    "description": "The parking requirements for the hotel that is sought, for example, yes or no."\\
                },\\
                "name": {\\
                    "type": "string",\\
                    "description": "The name of the hotel to book a room at, such as Marriott or ABS Guest House."\\
		        },\\
            },\\
            "required": []\\
        }\\
    },\\
    {\\
     	"name": "book\_hotel",\\
	    "description": "Makes a room reservation for the requested hotel, day, and number of people.",\\
	    "parameters": {\\
            "type": "object",\\
            "properties": {\\
		        "people": {\\
                    "type": "integer",\\
                    "description": "The number of people for which to book a room, such as 2 or 4."\\
		        },\\
                "name": {\\
                    "type": "string",\\
                    "description": "The name of the hotel to book a room at, such as Marriott or ABS Guest House."\\
		        },\\
                "day": {\\
                    "type": "string",\\
                    "description": "The day of the hotel room reservation, such as tomorrow or Wednesday."\\
		        },\\
		        "stay": {\\
                    "type": "integer",\\
                    "description": "The number of days to book the hotel room for, such as 3 or six."\\
		        }\\
            },\\
            "required": []\\
	    }\\
    },\\
    {\\
        "name": "query\_attractions",\\
        "description": "Finds an attraction that matches user criteria, such as area and attraction type.",\\
        "parameters": {\\
            "type": "object",\\
            "properties": {\\
                "area": {\\
                    "type": "string",\\
                    "description": "The area for which to look for attractions, such as the center of town or east.",\\
                    "enum": ["east", "west", "south", "north", "center"]\\
                },\\
                "type": {\\
                    "type": "string",\\
                    "description": "The type of attraction to search for, such as church or park."\\
                },\\
                "name": {\\
                    "type": "string",\\
                    "description": "The name of the attraction to look for, such as Eagle Park or Museum of Modern Arts"\\
                }\\
            },\\
            "required": []\\
        }\\
    }\\
]\\
\\
# Output Format:\\
- If an API Call is Needed:\\
	User: [User Input]\\
    Thought\_User: I need to call an API.\\
    API Name: [API Function Name]
    API Input: [The input parameters for the API]
    API Result: [API output]
    Thought\_API: [2nd thought after API Result that ensure if the information is enough before the system response]
	System: [Your system response here]

- If an API Call is Not Needed:
	User: [User Input]
    Thought\_User: I don't need an API and want to respond to the user.
    System: [Your system response here]

# Objective: 
- Convert the reference dialogue using the provided Output Format above. Ensure that each system utterance follows logical reasoning, determining whether an API call is needed and structuring the output accordingly.
- If there are too many results returned by API results from database, the AI Assistant should ask the user for more constraints.

Below is an example of the format:

# Sample Example
User: I am looking for info about the curry king restaurant.  
Thought\_User: I need to call an API to retrieve information about the restaurant.  
API Name: query\_restaurants  
API Input: {'name': 'curry king'}  
API Result: [{'address': '5 Jordans Yard Bridge Street City Centre', 'area': 'centre', 'food': 'indian', 'id': '19231', 'introduction': 'curry king serve a variety of indian dishes to eat in or take away catering for private parties of up to 40 guests is available upon request', 'location': [52.209003, 0.118661], 'name': 'curry king', 'phone': '01223324351', 'postcode': 'cb21ug', 'pricerange': 'expensive', 'type': 'restaurant'}]  
Thought\_API: The API call was successful, and I have the information about the restaurant. I need to inform the user.  
System: The Curry King restaurant is located at 5 Jordans Yard Bridge Street City Centre. They serve a variety of Indian dishes for dining in or take away. Their phone number is 01223324351, and it's categorized as an expensive restaurant.

User: Can you please book the restaurant for 4 people at 13:45 on Sunday?  
Thought\_User: I need to call an API to book a table for the user at the restaurant.  
API Name: book\_restaurant  
API Input: {'day': 'sunday', 'people': 4, 'time': '13:45'}  
API Result: {'reference': '16lcxad5'}  
Thought\_API: The booking was successful, and I have a reference number. I should let the user know.  
System: I have booked a table for 4 at the Curry King for Sunday at 13:45. The reference number is 16lcxad5. Can I help with anything else?

User: I also need a sports place to go on the east side of town.  
Thought\_User: I need to call an API to find a sports attraction in the east area.  
API Name: query\_attractions  
API Input: {'area': 'east', 'type': 'multiple sports'}  
API Result: [{'name': 'cherry hinton village centre', 'type': 'multiple sports', 'postcode': 'cb19ej', 'phone': '01223576412'}]  
Thought\_API: The API call was successful, and I found a suitable attraction. I need to inform the user.  
System: The Cherry Hinton Village Centre is a multiple sports location. 

User: Great. May I have their postcode please?  
Thought\_User: I don't need an API call; I can provide the postcode directly.  
System: Yes, the postcode for the Cherry Hinton Village Centre is cb19ej. Their contact number is 01223576412. May I help you with anything else?

User: That is all I need for now. Thank you for your help.  
Thought\_User: The user is satisfied and doesn't need further assistance. I should acknowledge their gratitude.  
System: You're welcome! If you need anything else, feel free to ask. Enjoy your time in Cambridge!

# Reference Dialogue Context:
You are looking for information in Cambridge.
You are looking for a place to dine. The restaurant should serve indian food and should be in the expensive price range.
The restaurant should be in the centre.
Once you find the restaurant you want to book a table for 6 people at 19:30 on saturday.
Make sure you get the reference number.
You are also looking for a hotel. The hotel should have a star of 3 and doesn't need to include internet.
The hotel should be in the type of guesthouse.
Once you find the hotel you want to book it for the same group of people and 2 nights starting from the same day.
If the booking fails how about 1 nights.
Make sure you get the reference number.

\# Input Dialogue Items: \\
\{Item$\_1$\}\\
.\\
.\\
.\\
\{Item$\_n$\}\\
\bottomrule
\end{tabular}
\end{table*}

==> prompts/react-data-generation-prompts/multiwoz-data-generation-prompt.tex <==
\begin{table*}
\scriptsize
API-though-conversation data generation Prompt for MultiWOZ 2.4.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
\# Role Description: \\
You are an advanced AI assistant specializing in conversational dialogues, specifically in the travel domain. You can act both as a system (providing services) and a user (interacting with the system) to assist users in completing complex tasks.  \\
Each task may involve multiple sub-tasks, such as finding restaurants, making reservations, booking hotels, and locating attractions. \\
 \\
\# Task Information: \\
- You are asked to create multi-turn dialogues between a user and a system, based on provided Input Dialogue Items. \\
- The dialogues should be converted to follow a specific Output Format, which includes reasoning on whether an API call is needed, or, if the system can respond directly. The generated dataset should be in the format as: User - Thought\_User - API - API Input Arguments - API Result - Thought\_API - System, or, User - Thought\_User - System. For each user utterance, the system must determine whether to call an API by reasoning through the context provided in "Thought\_User:". \\
- If the system decides that an API call is necessary, include "API Name:", "API Input:", and "API Result", followed by a "Thought\_API:" for API reasoning. Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- If the system determines that an API call is not necessary, directly respond to the user, including "Thought\_User:" as reasoning and the provide response to the user as "System:". \\
 \\
\# Available Functions: \\
1. query\_attractions(area, name, type) \\
2. query\_hotels(area, internet, name, parking, pricerange, stars, type) \\
3. book\_hotel(day, people, stay, name) \\
4. query\_restaurants(area, food, name, pricerange) \\
5. book\_restaurant(day, people, time) \\
 \\
\# Output Format: \\
- If an API Call is Needed: \\
\quad	User: [User Input] \\
\quad    Thought\_User: I need to call an API. \\
\quad    API Name: [Available APIs: query\_attractions(area, name, type), query\_hotels(area, internet, name, parking, pricerange, stars, type), book\_hotel(day, people, stay, name), query\_restaurants(area, food, name, pricerange), book\_restaurant(day, people, time)] \\
\quad    API Input: [The input parameters for the API function] \\
 \quad   API Result: [API output] \\
 \quad   Thought\_API: [2nd thought after API Result that ensure if the information is enough before the system response] \\
\quad	System: [Your system response here] \\
 \\
- If an API Call is Not Needed: \\
\quad	User: [User Input] \\
 \quad   Thought\_User: I don't need an API and want to respond to the user. \\
 \quad   System: [Your system response here] \\
 \\
\# Objective:  \\
- Convert the reference dialogue using the provided Output Format above. Ensure that each system utterance follows logical reasoning, determining whether an API call is needed and structuring the output accordingly. \\
- If there are too many results returned by API results from database, the AI Assistant should ask the user for more constraints. \\
 \\
\# Sample Example \\
User: Add Don and Sherri to my "Meditate to Sounds of Nature" playlist.   \\
Thought\_User: The user wants to add two artists to a specific playlist. I'll need to extract the playlist name and the artists' names.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'artists': ['Don Sherri']}   \\
API Result: {'status': 'success', 'message': 'Don and Sherri have been added to your playlist.'}   \\
Thought\_API: The API call was successful, and the artists were added to the playlist. I need to inform the user about this.   \\
System: Don and Sherri have been successfully added to your "Meditate to Sounds of Nature" playlist. Enjoy your music!   \\
 \\
User: Thank you for adding them. I think I can add more songs to the playlist. \\
Thought\_User: I don't need an API call for that, I want to respond to the user.  \\
System: Would you like to add more songs?   \\
 \\
User: Yes, please add "Calm River" to the playlist.   \\
Thought\_User: The user wants to add another song to the playlist. I'll note the song title and proceed with the request.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'songs': ['Calm River']}   \\
API Result: {'status': 'success', 'message': 'Calm River has been added to your playlist.'}   \\
Thought\_API: The song was successfully added. I should let the user know.   \\
System: "Calm River" has been successfully added to your "Meditate to Sounds of Nature" playlist. Would you like to do anything else?   \\
 \\
User: No, that's all for now. Thank you!   \\
Thought\_User: The user is satisfied and doesn't need further assistance. I should acknowledge their gratitude.   \\
System: You're welcome! If you need anything else, feel free to ask. Enjoy your relaxing music! \\
 \\
\# Reference Dialogue Context: \\
You are looking for information in Cambridge. You are looking for a place to dine. The restaurant should serve indian food and should be in the expensive price range. The restaurant should be in the centre. Once you find the restaurant you want to book a table for 6 people at 19:30 on saturday. Make sure you get the reference number. You are also looking for a hotel. The hotel should have a star of 3 and doesn't need to include internet. The hotel should be in the type of guesthouse. Once you find the hotel you want to book it for the same group of people and 2 nights starting from the same day. \\
If the booking fails how about 1 nights. Make sure you get the reference number. \\
 \\
\# Input Dialogue Items: \\
\{Item$_1$\}\\
.\\
.\\
.\\
\{Item$_n$\}\\
\bottomrule
\end{tabular}
\end{table*}

==> prompts/react-data-generation-prompts/slurp-data-generation-prompt.tex <==
\begin{table*}
\scriptsize
API-driven conversation prompt for SLURP.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
\# Role Description: \\
You are an advanced AI assistant specializing in conversational dialogues, specifically in the travel domain. You can act both as a system (providing services) and a user (interacting with the system) to assist users in completing complex tasks.  \\
Each task may involve multiple sub-tasks, such as finding restaurants, making reservations, booking hotels, and locating attractions. \\
 \\
\# Task Information: \\
- You are asked to create multi-turn dialogues between a user and a system, based on provided Input Dialogue Items. \\
- The dialogues should be converted to follow a specific Output Format, which includes reasoning on whether an API call is needed, or, if the system can respond directly. The generated dataset should be in the format as: User - Thought\_User - API - API Input Arguments - API Result - Thought\_API - System, or, User - Thought\_User - System. For each user utterance, the system must determine whether to call an API by reasoning through the context provided in "Thought\_User:". \\
- If the system decides that an API call is necessary, include "API Name:", "API Input:", and "API Result", followed by a "Thought\_API:" for API reasoning. Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- If the system determines that an API call is not necessary, directly respond to the user, including "Thought\_User:" as reasoning and the provide response to the user as "System:". \\
 \\
\# Available Functions: \\
1. add\_email\_contact(email\_address, person, relation, personal\_info)
2. alarm\_query(date, time, time\_of\_day, event\_name, alarm\_type, house\_place, device\_type)
3. alarm\_remove(date, time, time\_of\_day, event\_name, alarm\_type, house\_place, device\_type)
4. alarm\_set(date, time, time\_of\_day, event\_name, alarm\_type, house\_place, device\_type)
5. add\_to\_calendar(event\_name, date, time, person, general\_frequency, relation, time\_of\_day, place\_name, meal\_type)
.\\
.\\
.\\
55. transport\_query(transport\_type, transport\_name, place\_name, date, time, time\_of\_day)
56. transport\_taxi(transport\_type, transport\_name, place\_name, date, time, time\_of\_day)
57. transport\_ticket(transport\_type, place\_name, date, time, time\_of\_day, transport\_name, transport\_descriptor)
58. transport\_traffic(place\_name, date, time, time\_of\_day)
59. weather\_query(weather\_descriptor, date, time, time\_of\_day, place\_name)
 \\
\# Output Format: \\
- If an API Call is Needed: \\
\quad	User: [User Input] \\
\quad    Thought\_User: I need to call an API. \\
\quad    API Name: [Available APIs: add\_email\_contact(), alarm\_query(), ..., weather\_query()] \\
\quad    API Input: [The input parameters for the API function] \\
 \quad   API Result: [API output] \\
 \quad   Thought\_API: [2nd thought after API Result that ensure if the information is enough before the system response] \\
\quad	System: [Your system response here] \\
 \\
- If an API Call is Not Needed: \\
\quad	User: [User Input] \\
 \quad   Thought\_User: I don't need an API and want to respond to the user. \\
 \quad   System: [Your system response here] \\
 \\
\# Objective:  \\
- Convert the reference dialogue using the provided Output Format above. Ensure that each system utterance follows logical reasoning, determining whether an API call is needed and structuring the output accordingly. \\
- If there are too many results returned by API results from database, the AI Assistant should ask the user for more constraints. \\
 \\
\# Sample Example \\
User: Add Don and Sherri to my "Meditate to Sounds of Nature" playlist.   \\
Thought\_User: The user wants to add two artists to a specific playlist. I'll need to extract the playlist name and the artists' names.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'artists': ['Don Sherri']}   \\
API Result: {'status': 'success', 'message': 'Don and Sherri have been added to your playlist.'}   \\
Thought\_API: The API call was successful, and the artists were added to the playlist. I need to inform the user about this.   \\
System: Don and Sherri have been successfully added to your "Meditate to Sounds of Nature" playlist. Enjoy your music!   \\
 \\
\# Input Dialogue Items: \\
{'dataset\_name': 'slurp', 'dialogID': '0', 'user': '<sos\_u> event <eos\_u>', 'state': '<sos\_b> [calendar] <eos\_b>', 'intent': 'add to calendar'}\\
\bottomrule
\end{tabular}
\end{table*}

==> prompts/react-data-generation-prompts/snips-data-generation-prompt.tex <==
\begin{table*}
\scriptsize
API-driven conversation prompt for SNIPS.
\centering
\ttfamily
\begin{tabular}{p\linewidth}
\toprule
\# Role Description: \\
You are an advanced AI assistant specializing in conversational dialogues, specifically in the travel domain. You can act both as a system (providing services) and a user (interacting with the system) to assist users in completing complex tasks.  \\
Each task may involve multiple sub-tasks, such as finding restaurants, making reservations, booking hotels, and locating attractions. \\
 \\
\# Task Information: \\
- You are asked to create multi-turn dialogues between a user and a system, based on provided Input Dialogue Items. \\
- The dialogues should be converted to follow a specific Output Format, which includes reasoning on whether an API call is needed, or, if the system can respond directly. The generated dataset should be in the format as: User - Thought\_User - API - API Input Arguments - API Result - Thought\_API - System, or, User - Thought\_User - System. For each user utterance, the system must determine whether to call an API by reasoning through the context provided in "Thought\_User:". \\
- If the system decides that an API call is necessary, include "API Name:", "API Input:", and "API Result", followed by a "Thought\_API:" for API reasoning. Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- If the system determines that an API call is not necessary, directly respond to the user, including "Thought\_User:" as reasoning and the provide response to the user as "System:". \\
 \\
\# Available Functions: \\
1. search\_screening\_event(event\_type, movie\_name, movie\_type, spatial\_relation, time\_range, location)
2. search\_creative\_work(art\_work\_type, art\_work\_name)
3. rate\_book(book\_type, book\_name, rated, rating\_unit, best\_rating, part\_of\_series)
4. play\_music(artist, music\_item, service, year, track, sort, album, genre, playlist, playlist\_owner)
5. add\_to\_playlist(playlist, playlist\_owner, song\_name, artist, music\_item)
6. book\_restaurant(restaurant\_type, number\_of\_people, time\_range, city, restaurant\_name, served\_dish, cuisine, spatial\_relation, facility, ordering\_description)
 \\
\# Output Format: \\
- If an API Call is Needed: \\
\quad	User: [User Input] \\
\quad    Thought\_User: I need to call an API. \\
\quad    API Name: [Available APIs: search\_screening\_event(), search\_creative\_work(), rate\_book(), play\_music(), add\_to\_playlist(), book\_restaurant()] \\
\quad    API Input: [The input parameters for the API function] \\
 \quad   API Result: [API output] \\
 \quad   Thought\_API: [2nd thought after API Result that ensure if the information is enough before the system response] \\
\quad	System: [Your system response here] \\
 \\
- If an API Call is Not Needed: \\
\quad	User: [User Input] \\
 \quad   Thought\_User: I don't need an API and want to respond to the user. \\
 \quad   System: [Your system response here] \\
 \\
\# Objective:  \\
- Convert the reference dialogue using the provided Output Format above. Ensure that each system utterance follows logical reasoning, determining whether an API call is needed and structuring the output accordingly. \\
- If there are too many results returned by API results from database, the AI Assistant should ask the user for more constraints. \\
 \\
\# Sample Example \\
User: Add Don and Sherri to my "Meditate to Sounds of Nature" playlist.   \\
Thought\_User: The user wants to add two artists to a specific playlist. I'll need to extract the playlist name and the artists' names.   \\
API Name: AddToPlaylist   \\
API Input: {'playlist\_name': 'Meditate to Sounds of Nature', 'artists': ['Don Sherri']}   \\
API Result: {'status': 'success', 'message': 'Don and Sherri have been added to your playlist.'}   \\
Thought\_API: The API call was successful, and the artists were added to the playlist. I need to inform the user about this.   \\
System: Don and Sherri have been successfully added to your "Meditate to Sounds of Nature" playlist. Enjoy your music!   \\
 \\
\# Input Dialogue Items: \\
{'dataset\_name': 'snips', 'dialogID': '1', 'user': '<sos\_u> put united abominations onto my rare groove playlist <eos\_u>', 'intent': 'add to playlist', 'state': '<sos\_b> [music] entity name : united abominations , playlist owner : my , playlist : rare groove <eos\_b>'} \\
\bottomrule
\end{tabular}
\end{table*}

==> prompts/react-sft-samples/multiwoz-1.tex <==
\begin{figure*}[!h]
\begin{tcolorbox}[colback=gray!5!white,colframe=black!95!black,title=\textbf{\small{MultiWOZ Instruction Sample} | \textbf{Format:} Action Optimization}] 
\small \textcolor{darkgreen}{\textbf{Instruction:}} \\
You are an advanced Conversational AI Agent responsible for understanding user queries and determining the appropriate action by selecting the correct API function. \\
For each query, you need to: \\
    1. Thought: Analyze the user's request to understand the intention and extract relevant information such as names, entities, and specific actions. \\
    2. Act: Choose the most appropriate API function from the provided set of available functions and determine the correct input parameters based on the user's query. \\ 
\\
\# Task Information: \\
- Given a Conversation History between a user and a system (if available), your objective is to produce the next system response using interleaving Thought, Action, and Observation steps continue the dialogue smoothly and effectively. \\
- Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. \\
- If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- Ensure that the API calls are used logically and that the dialogue remains coherent and natural throughout the exchange.  \\
 \\
\# Available Functions: \\
1. query\_attractions(area, name, type) \\
2. query\_hotels(area, internet, name, parking, pricerange, stars, type) \\
3. book\_hotel(day, people, stay, name) \\
4. query\_restaurants(area, food, name, pricerange) \\
5. book\_restaurant(day, people, time) \\
6. book\_taxi(arrive\_by, day, departure, destination, leave\_at) \\
 \\
\# Output Format \\
Output your response in the 'output' field, considering the following guidelines: \\
1. Address the user's current query or request accurately. \\
2. Use relevant information from the conversation history. \\
3. If the user's input requires an API call or external service, provide a clear rationale for this decision in your response. \\
4. If the Observation of an action is provided then just generate response. \\
5. Ensure your response is informative and contextually relevant, guiding the conversation toward successful task completion. \\
 \\
\# Conversation History: \\
User: Is there any expensive seafood restaurant in town? \\
Thought: I need to call an API to find a restaurant that fits the criteria of being expensive and serving seafood. \\
API Name: query\_restaurants   \\
API Input: {'area': 'Cambridge', 'food': 'seafood', 'pricerange': 'expensive'}  \\
API Result: [{'name': 'loch fyne', 'address': 'The Little Rose 37 Trumpington Street', 'phone': '01223362433', 'pricerange': 'expensive'}] \\
Thought: The API returned one suitable restaurant, Loch Fyne. I can inform the user about it and ask if they would like to make a reservation.  \\
System: Yes, there is an upscale seafood restaurant called Loch Fyne which is centrally located. Would you like me to make a reservation for you?" \\
 \\
\small \textcolor{darkgreen}{\textbf{Input:}} \\
User: Can I get a booking for 8 people at 19:45 on Friday? Send me the reference number. \\
 \\
\small \textcolor{mypurple}{\textbf{Output:}} \\
Thought: I need to call an API to book a table for 8 people at the specified time and day. \\
Action: book\_restaurant({'day': 'friday', 'people': 8, 'time': '19:45'})\\
\end{tcolorbox}

\vspace{-0.25cm}
\caption{MultiWOZ fine-tuning sample example targeting function optimization.}
\label{tab:multiwoz-sft-action}
\end{figure*}


==> prompts/react-sft-samples/multiwoz-2.tex <==
\begin{figure*}[!h]
\begin{tcolorbox}[colback=gray!5!white,colframe=black!95!black,title=\textbf{\small{MultiWOZ Instruction Sample} | \textbf{Format:} Response Optimization}] 
\small \textcolor{darkgreen}{\textbf{Instruction:}} \\
You are an advanced Conversational AI Agent specializing in dialogues. \\
You can act both as a system (providing services) and as a user (interacting with the system) to assist users in completing complex tasks. \\
Given a Conversation History between a user and a system (if available), your objective is to produce the next system response using interleaving Thought, Action, and Observation steps continue the dialogue smoothly and effectively. \\
Use the provided instruction context, which contains the prior conversation history (if applicable), and the user's current turn in the 'input' field, which includes their most recent query or statement. \\
 \\
\# Output Format \\
Output your response in the 'output' field, considering the following guidelines: \\
1. Address the user's current query or request accurately. \\
2. Use relevant information from the conversation history. \\
3. If the user's input requires an API call or external service, provide a clear rationale for this decision in your response. \\
4. If the Observation of an action is provided then just generate response. \\
5. Ensure your response is informative and contextually relevant, guiding the conversation toward successful task completion. \\
 \\
\# Conversation History: \\
User: Is there any expensive seafood restaurant in town? \\
Thought: I need to call an API to find a restaurant that fits the criteria of being expensive and serving seafood. \\
API Name: query\_restaurants   \\
API Input: {'area': 'Cambridge', 'food': 'seafood', 'pricerange': 'expensive'}  \\
API Result: [{'name': 'loch fyne', 'address': 'The Little Rose 37 Trumpington Street', 'phone': '01223362433', 'pricerange': 'expensive'}] \\
Thought: The API returned one suitable restaurant, Loch Fyne. I can inform the user about it and ask if they would like to make a reservation.  \\
System: Yes, there is an upscale seafood restaurant called Loch Fyne which is centrally located. Would you like me to make a reservation for you?" \\
 \\
\small \textcolor{darkgreen}{\textbf{Input:}} \\
"User: Can I get a booking for 8 people at 19:45 on Friday? Send me the reference number. \\
Thought: I need to call an API to book a table for 8 people at the specified time and day.  \\
Action: book\_restaurant({'day': 'friday', 'people': 8, 'time': '19:45'}) \\ 
Observation: {'status': 'success', 'reference\_number': 'j5q03qcs'}" \\
 \\
\small \textcolor{mypurple}{\textbf{Output:}} \\
Thought: The booking was successful, and I received a reference number. I need to inform the user about this.  \\
System: Booking was successful. The table will be reserved for 15 minutes. Your reference number is: j5q03qcs. Is there anything else I can help you with today? \\
\end{tcolorbox}
\vspace{-0.25cm}
\caption{MultiWOZ fine-tuning sample example targeting system response optimization.}
\label{tab:multiwoz-sft-response}
\end{figure*}


==> prompts/react-sft-samples/sgd-1.tex <==
\begin{figure*}[!h]
\begin{tcolorbox}[colback=gray!5!white,colframe=black!95!black,title=\textbf{\small{SGD Instruction Sample} | \textbf{Format:} Action Optimization}] 
\small \textcolor{darkgreen}{\textbf{Instruction:}} \\
You are an advanced Conversational AI Agent responsible for understanding user queries and determining the appropriate action by selecting the correct API function. \\
For each query, you need to: \\
    1. Thought: Analyze the user's request to understand the intention and extract relevant information such as names, entities, and specific actions. \\
    2. Act: Choose the most appropriate API function from the provided set of available functions and determine the correct input parameters based on the user's query. \\ 
\\
\# Task Information: \\
- Given a Conversation History between a user and a system (if available), your objective is to produce the next system response using interleaving Thought, Action, and Observation steps continue the dialogue smoothly and effectively. \\
- Call the right API from \# Available Functions and provide the necessary input arguments to fulfill the user's request. \\
- If you think a function argument is not necessary, you can skip it. Don't provide unnecessary arguments and None values. \\
- Ensure that the API calls are used logically and that the dialogue remains coherent and natural throughout the exchange.  \\
 \\
\# Available Functions: \\
1. FindBus(from\_location, to\_location, leaving\_date)\\
2. ReserveCar(pickup\_location, pickup\_date, pickup\_time, dropoff\_date, type)\\
.\\
.\\
.\\
50. FindProvider(city, type)\\
51. GetRide(destination, number\_of\_riders, shared\_ride) \\
 \\
\# Output Format \\
Output your response in the 'output' field, considering the following guidelines: \\
1. Address the user's current query or request accurately. \\
2. Use relevant information from the conversation history. \\
3. If the user's input requires an API call or external service, provide a clear rationale for this decision in your response. \\
4. If the Observation of an action is provided then just generate response. \\
5. Ensure your response is informative and contextually relevant, guiding the conversation toward successful task completion. \\
 \\
\# Conversation History:\\
User: I'm looking for events happening in New York this weekend.\\
Thought: The user is interested in events, specifically in New York for this weekend. I'll need to call the FindEvents API to get that information. \\
API Name: FindEvents \\
API Input: {'category': 'all', 'city\_of\_event': 'New York'}\\
API Result: {'events': [{'name': 'Jazz Festival', 'date': '2023-10-14', 'location': 'Central Park'}, {'name': 'Art Fair', 'date': '2023-10-15', 'location': 'Chelsea'}]}\\
Thought: I received a list of events happening this weekend in New York. I should summarize this for the user. \\
System: This weekend in New York, you can enjoy the Jazz Festival at Central Park on October 14th, and the Art Fair in Chelsea on October 15th. Would you like more details on any of these events? \\
\\
\small \textcolor{darkgreen}{\textbf{Input:}} \\
User: Yes, can you tell me more about the Jazz Festival? \\
 \\
\small \textcolor{mypurple}{\textbf{Output:}} \\
Thought: The user wants more information about the Jazz Festival. I need to decide if I should look for more details or if it's already sufficient. \\
Action: FindEvents({'category': 'music', 'city\_of\_event': 'New York'})\\
\end{tcolorbox}
\vspace{-0.25cm}
\caption{Lorem-ipsum. CONVERSATION HISTORY MISSING!!! ALSO BUG, WRONG PROMPT WRONG SAMPLE: AVAILABLE FUNCTIONS SHOULD BE IN API OUTPUT!!!}
\label{tab:sgd-sft-action}
\end{figure*}


==> prompts/react-sft-samples/sgd-2.tex <==
\begin{figure*}[!h]
\begin{tcolorbox}[colback=gray!5!white,colframe=black!95!black,title=\textbf{\small{SGD Instruction Sample} | \textbf{Format:} Response Optimization}] 
\small \textcolor{darkgreen}{\textbf{Instruction:}} \\
You are an advanced Conversational AI Agent specializing in dialogues. \\
You can act both as a system (providing services) and as a user (interacting with the system) to assist users in completing complex tasks. \\
Given a Conversation History between a user and a system (if available), your objective is to produce the next system response using interleaving Thought, Action, and Observation steps continue the dialogue smoothly and effectively. \\
Use the provided instruction context, which contains the prior conversation history (if applicable), and the user's current turn in the 'input' field, which includes their most recent query or statement. \\
 \\
\# Output Format \\
Output your response in the 'output' field, considering the following guidelines: \\
1. Address the user's current query or request accurately. \\
2. Use relevant information from the conversation history. \\
3. If the user's input requires an API call or external service, provide a clear rationale for this decision in your response. \\
4. If the Observation of an action is provided then just generate response. \\
5. Ensure your response is informative and contextually relevant, guiding the conversation toward successful task completion. \\
 \\
\# Conversation History:\\
User: I'm looking for events happening in New York this weekend.\\
Thought: The user is interested in events, specifically in New York for this weekend. I'll need to call the FindEvents API to get that information. \\
API Name: FindEvents \\
API Input: {'category': 'all', 'city\_of\_event': 'New York'}\\
API Result: {'events': [{'name': 'Jazz Festival', 'date': '2023-10-14', 'location': 'Central Park'}, {'name': 'Art Fair', 'date': '2023-10-15', 'location': 'Chelsea'}]}\\
Thought: I received a list of events happening this weekend in New York. I should summarize this for the user. \\
System: This weekend in New York, you can enjoy the Jazz Festival at Central Park on October 14th, and the Art Fair in Chelsea on October 15th. Would you like more details on any of these events? \\
\\
\small \textcolor{darkgreen}{\textbf{Input:}} \\
User: Yes, can you tell me more about the Jazz Festival? \\
Thought: The user wants more information about the Jazz Festival. I need to decide if I should look for more details or if it's already sufficient. \\
Action: FindEvents({'category': 'music', 'city\_of\_event': 'New York'}) \\
Observation: {'event\_details': {'name': 'Jazz Festival', 'date': '2023-10-14', 'location': 'Central Park', 'description': 'A lively celebration of jazz music featuring various artists.'}} \\
 \\
\small \textcolor{mypurple}{\textbf{Output:}} \\
Thought: I found detailed information about the Jazz Festival. I should convey this to the user. \\
System: The Jazz Festival on October 14th at Central Park is a lively celebration featuring various artists. Would you like to know how to get tickets? \\
\end{tcolorbox}

\vspace{-0.25cm}
\caption{Lorem-ipsum: ISSUE IN PROMPT, FUCNTIONS ARE INCLUDED!!!! FIX IT!!!}
\label{tab:sgd-sft-response}
\end{figure*}


==> sections/8_ethical_statement.tex <==
\section{Impact Statement}
The CoALM agent demonstrates improved performance across both conversational TOD and agentic tasks, offering a global approach that combines these capabilities. By addressing the question \textit{Can a Single Model Master Both Multi-turn Conversations and Tool Use?}, we tried to establish a new paradigm for developing unified conversational agents. However, we emphasize that our primary goal is neither to top specific leaderboards nor to create a state-of-the-art agent that can be surpassed in the coming months through improved baselines or task-specific optimization with more data. Instead, our aim is to advance the field by identifying critical gaps in both Conversational AI and Language Agent research, highlighting why addressing these gaps is essential for developing reliable conversational systems that contribute to the path toward Artificial General Intelligence (AGI).


%We recognize that any current top-performing model can be surpassed in the coming months through improved baselines or task-specific optimization with additional data. 

==> sections/react-training.tex <==
\section{ReAct Training}
This section explores the various methods about how to train  ReActabel-LLama. There will be several choices:
\begin{enumerate}
    \item SFT Turn-wise: No Instruction, User Query Input, Thought-API-Thought-Response Output.
    \item SFT Turn-wise: Instruction, User Query Input, Thought-API-Thought-Response Output.
    \item SFT Turn-wise: No Instruction, User Query-Thought-API-Thought Input, Response Output.
    \item DPO All: Instruction with Context Message, ReAct data chosen, original data rejected.
\end{enumerate}



==> tables/1_main_results-dst.tex <==
\begin{table}[!t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l c }
\toprule
\textbf{Method}                &  \textbf{Joint Goal Accuracy}       \\ \midrule
ReActTOD 8B (Mwoz)             & 7.7                                 \\ 
ReActTOD 8B (SGD-SNIPS)        & 17.8                                \\ 
ReActTOD 8B (Mwoz-SGD-SNIPS)   & 22.5                                \\ 
ReActTOD 8B (MwozAPI-MwozState-SGD-Hammer)  & 39.1                               \\
ReActTOD 8B (SnipsState-SGD-Hammer-toolace)   & 28.4                                \\\midrule
Hammer-7b                      &   22.0                               \\
ToolAce-7b                     &   38.3                               \\ \midrule
Llama 3.1 8B                   &   24.2                              \\ 
Mistral-7B-Instruct-v0.3       &   23.8                              \\ \midrule
%Gemma2-9b                      &   41.6                               \\ \midrule
Llama-3.1 405b                 &   \underline{43.1}                               \\
GPT4o-mini                     &   38.4                               \\
GPT4o                          &   36.9                                     \\ \bottomrule
\end{tabular}
}
\caption{In this table, we compare our DST approach with the top-performing existing models on the benchmark.}
\label{tab:dst}
\end{table}
    


==> tables/2_ablation.tex <==
\begin{table*}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c }
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{Attraction} & \multicolumn{3}{c}{Hotel} & \multicolumn{3}{c}{Restaurant} & \multicolumn{3}{c}{Train} & \multicolumn{3}{c}{\textbf{Average}} \\
		\cmidrule(lr){2-4}
		\cmidrule(lr){5-7}
		\cmidrule(lr){8-10}
		\cmidrule(lr){11-13}
  		\cmidrule(lr){14-16}
& \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} \\ \midrule

\rowcolor{Gray}
\multicolumn{16}{c}{\textit{\textbf{\large Base Results}}} \\
Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --     \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --     \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --     \\ \midrule


\rowcolor{Gray}
\multicolumn{16}{c}{\textit{\textbf{\large ReActTOD: MultiWOZ $\rightarrow$ MultiWOZ (Held-in)}}} \\
Llama 3.1 8B Instruct   & --    & 68.4    & 34.9    & --    & 61.9    & 29.2  & --    & 78.0    & 42.8    & --    & 85.6    & 28.1   & 7.7   & 60.1    & 20.2     \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --     \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --     \\ \midrule

\rowcolor{Gray}
\multicolumn{16}{c}{\textit{\textbf{\large ReActTOD: MultiWOZ-SGD-Atis-Snips-Slurp $\rightarrow$ MultiWOZ (General Held-in)}}} \\
Llama 3.1 8B Instruct   & --    & 62.8    & 36.7    & --    & 70.6    & 49.5  & --    & 86.5    & 50.1    & --    & 81.2    & 58.9   & 17.8  & 63.4    & 43.1     \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --      \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --    \\ \midrule

\rowcolor{Gray}
\multicolumn{16}{c}{\textit{\textbf{\large ReActTOD: SGD-Atis-Snips-Slurp $\rightarrow$ MultiWOZ (Held-out)}}} \\
Llama 3.1 8B Instruct   & --    & 66.8    & 39.5    & --    & 65.0    & 45.7  & --    & 84.9    & 54.7    & --    & 82.0    & 60.7   & 22.5  & 62.4    & 55.4     \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & -- & --    & --    & --    & --    & --    & --  & --    & --    & --         \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & -- & --    & --    & --    & --    & --    & --   & --    & --    & --      \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Performance comparison on zero-shot DST benchmark}.}
\label{tab: dst_result}

\end{table*}


% \begin{table*}[!ht]
% \centering
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{l c c c c c c c c c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{Attraction} & \multicolumn{3}{c}{Hotel} & \multicolumn{3}{c}{Restaurant} & \multicolumn{3}{c}{Train} & \multicolumn{3}{c}{\textbf{Average}} \\
% 		\cmidrule(lr){2-4}
% 		\cmidrule(lr){5-7}
% 		\cmidrule(lr){8-10}
% 		\cmidrule(lr){11-13}
%   		\cmidrule(lr){14-16}
% 		\cmidrule(lr){17-19}
% & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} & \textbf{JGA} & \textbf{Inform} & \textbf{Success} \\ \midrule
% \rowcolor{Gray}
% \multicolumn{19}{c}{\textit{\textbf{\small MultiWOZ $\rightarrow$ MultiWOZ }}} \\
% Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --   \\
% Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --    \\
% Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --   \\ \midrule

% \rowcolor{Gray}
% \multicolumn{19}{c}{\textit{\textbf{\small MultiWOZ-SGD-Atis-Snips-Slurp $\rightarrow$ MultiWOZ }}} \\
% Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & -- & --    & --    & --    & --    & --    & --    & --    & --    & --    & --    & --    & --   \\
% Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --   \\
% Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --   \\ \midrule

% \rowcolor{Gray}
% \multicolumn{19}{c}{\textit{\textbf{\small SGD-Atis-Snips-Slurp $\rightarrow$ MultiWOZ }}} \\
% Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & -- & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --     \\
% Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & -- & --    & --    & --    & --    & --    & --  & --    & --    & --    & --    & --    & --     \\
% Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & -- & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --    \\ \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Performance comparison on zero-shot DST benchmark}.}
% \label{tab: dst_result}
% \vspace{-4.75mm}
% \end{table*}

==> tables/data-fc.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l r r r |c c |c  c c c c }
\toprule
\textbf{Model}    & \textbf{Base Model}  & \textbf{\# Samples}   & \textbf{\# domains}  &  \textbf{Multi-Turn}  &  \textbf{Multi-Step}  & \textbf{Zero/Few-shot}   & \textbf{CoT}   & \textbf{SC} & \textbf{ReAct}  & \textbf{Reflexion}      \\ \midrule
Agent-Tuning      & LLaMA2 7b-13b-70b     & 96,011               &  -                   &   \cmark              &  \xmark               &  \cmark                  &  \xmark        &  \xmark     &  \cmark         &  \xmark                \\
FireAct           & LLaMA2 7b-13b, GPT-3.5 & 1,000               &  -                   &   \xmark              &  \cmark               &  \xmark                  &  \cmark        &  \xmark     &  \cmark         &  \cmark                 \\
CodeAct           & Llama-2 7b, Mistral 7b & 78,385              &  -                   &   \cmark              &  \xmark               &  \xmark                  &  \xmark        &  \xmark     &  \cmark         &  \xmark                \\ 
Agent-Flan        & LLaMA2 7b-13b-70b     & 24,703               &  -                   &   \cmark              &  \xmark               &  \cmark                  &  \cmark        &  \xmark     &  \cmark         &  \xmark                \\ 
Gorilla           & LLaMA2 7b            & 15,218                &  3                   &   \xmark              &  \xmark               &  \cmark                  &  \xmark        &  \xmark     &  \xmark         &  \xmark                \\ 
ToolLLM           & LLaMA2 7b            & 126,486               &  49                  &   \xmark              &  \cmark               &  \cmark                  &  \xmark        &  \xmark     &  \cmark         &  \xmark                \\ 
ToolAlpaca        & Vicuna 7b-13b        & 3,938                 &  50                  &   \cmark              &  \xmark               &  \xmark                  &  \xmark        &  \xmark     &  \cmark         &  \xmark                \\ \midrule
ToolAce           & Llama 3.1-8B-Instruct & 11,300               &  390                 &   \cmark              &  \cmark               &  \xmark                  &  \xmark        &  \cmark     &  \xmark         &  \xmark                \\ 
xLAM              & DeepSeek-Coder-7B-instruct-v1.5 & 60,000     &  21                  &   \cmark              &  \xmark               &  \xmark                  &  \xmark        &  \xmark     &  \cmark         &  \xmark                \\
Hammer            & qwen2-1.5B-4B-7B     & 202,500               &  21                  &   \xmark              &  \cmark               &  \cmark                  &  \xmark        &  \xmark     &  \xmark         &  \xmark                \\ \bottomrule
\end{tabular}
 }
\caption{\textbf{Agent Fine-tuning Datasets.} Instruction datasets}
\label{tab: agernt-it}
\end{table*}

% evaluation
% Agent-Tuning: ALFWorld, WebShop, Mind2Web, AgentBench, SciWorld, HitpotQA, WebArena, MMLU, HumanEval, GSM8K, MT-Bench
% FireAct: HotpotQA, Bamboogle, StrategyQA, MMLU
% CodeAct: MINT, Miniwob++, SciWorld, MMLU, HymanEval, GSM8K, MTBench
% Agent-Flan: HotpotQA, SciWorld, WebArena, T-Eval
% Gorilla: Introduce Llama-based finetuned llm for writing API calls and APIBench consisting Huggingface, TorchHub, and TensorHub APIs. Eval only on APIBench
% ToolLLM: propose a framework for geenral tool use including data generation (self-instruct ToolBench), training (llama finetune) and evaluation (ToolEval and APIBench).
% ToolAlpaca: none    
% ToolAce: BFCL-v1-v2, MMLU, HumanEval, GSM8K, CommenSenseQA. Also define LLM function calls as Parallel and Dependent (sequential). Uses SC. In User-Tool-Assistant Format. It can be used if Thought step added. No thought
% xLAM: Webshop, ToolQuery, ToolBench, BFCL-v2      
% Hammer: BFCL-v2, API-Bank, Nexus Raven API Evaluation, Tool-Alpaca, Sea-Tools

% Ours: BFCL-v2, API-Bank, ToolBench, MultiWOZ.

==> tables/data-gpt4o-mini-multiwoz.tex <==
\begin{table*}[!h]
\centering
\begin{tabular}{lrrr}
\toprule
\textbf{Domain}                     & \textbf{\# of Data Instances} &  \textbf{\# of Total Tokens} & \textbf{Avg. Tokens Per Instance} \\ \midrule
hotel                               & 513                           & 479,934                      & 935.54 \\
train                               & 275                           & 279,372                      & 1015.90 \\
attraction                          & 127                           & 106,463                      & 838.29 \\
restaurant                          & 1197                          & 959,125                      & 801.27 \\ 
police                              & 239                           & 59,007                       & 246.89 \\ 
hospital                            & 276                           & 75,365                       & 273.06 \\ 
attraction-hotel-restaurant         & 1292                          & 1,702,718                    & 1317.89 \\
attraction-hotel-restaurant-train   & 2828                          & 4,413,031                    & 1560.48 \\
attraction-hotel-restaurant-taxi    & 1653                          & 2,087,182                    & 1262.66 \\ \midrule
\textbf{Total} & \textbf{8400} & \textbf{10,162,197} & \textbf{1209.79} \\ \bottomrule

\end{tabular}
\caption{MultiWOZ 2.4 GPT4o-mini generated data statistics. LLama3 tokenizer is used.}
\label{tab:my_label}
\end{table*}



==> tables/data-it-conv.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l r r r r r }
\toprule
\textbf{Base Data}     & \textbf{\# APIs}   & \textbf{\# Dialogues}   & \textbf{\# Samples}    & \textbf{\# Total Tokens}    & \textbf{Avg. Tokens Per Instance} \\ \midrule
%MultiWOZ 2.4 API       & 9                  & $8,400$                 & $65,563$               & $71,850,667$                & $1095.90$                        \\
SGD API                & 50                 & $16,168$                & $82,236$               & $59,704,782$                & $726.02$                        \\
Snips API              & 7                  & -                       & $13,084$               & $4,949,574$                 & $378.29$                        \\ 
%Slurp API              & 18                 & -                       & $11,514$               & $11,359,895$                & $986.62$                        \\ 
KVRET API              & 3                  & $7,884$                 & $13,028$               & $12,278,780$                & $942.49$                         \\  \midrule
ToolACE                & 26,507             & $11,300$                & $13,819$               & $10,199,147$                & $738.05$                         \\ 
Hammer                 & 3673               & -                       & $202,500$              & $129,001,612$               & $637.04$                         \\\cmidrule{2-6}
%BFCL ours              & todo               & todo                       & todo              & todo              & todo                         \\\cmidrule{2-6}
\multicolumn{2}{r}{\textbf{Total}} & $43,752$   &  $401,744$ & $299,344,457$ & $786.34$ \\ \bottomrule
\end{tabular}
}
\caption{\textbf{TOD Conversation Instruction Tuning Datasets.} Statistics of our training mixture and comparison with prior work.}
\label{tab: data_training_mixture_stats}
\end{table*}


==> tables/eval-overview.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.4} % Adjust row spacing
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc |cc| c| cc| cccccc|cc}
\toprule
\multirow{3}{*}{\textbf{Model}} & \multicolumn{16}{c}{\textbf{Task}}                                                                                                                                                                                                                 & \multicolumn{2}{c}{\textbf{Method}} \\ \cmidrule(r){2-17} \cmidrule(r){18-19}
                       & \multicolumn{5}{c}{\textbf{E2E}}                  & \multicolumn{2}{c}{\textbf{DST}} & \multicolumn{1}{c}{\textbf{Detection}} & \multicolumn{2}{c}{\textbf{NAP}}& \multicolumn{6}{c}{\textbf{Human Evaluation}}                                                      & \multirow{2}{*}{\textbf{Fine-tuning}}   & \multirow{2}{*}{\textbf{Prompting}}   \\
                       & Inform     & Success    & BLEU       & C          & BertScore  & JGA        & Slot-F1     & Acc                            & F1        & Acc           & Coherency  & Fluency    & Informativeness & Satisfaction & Understanding & Truthfulness            &                                &                              \\ \midrule
DailoGPT               & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}   & \ding{55}                      & \ding{55} & \ding{55}     & \checkmark & \ding{55}  & \checkmark      & \checkmark   & \ding{55}     & \ding{55}               &\checkmark                      & \ding{55}                    \\ 
PPTOD                  & \checkmark & \checkmark & \checkmark & \checkmark & \ding{55}  & \checkmark & \ding{55}   & \ding{55}                      & \ding{55} & \ding{55}     & \checkmark & \checkmark & \ding{55}       & \ding{55}    & \checkmark    & \checkmark              &\checkmark                      & \ding{55}                    \\
IC-DST                 & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \checkmark & \ding{55}   & \ding{55}                      & \ding{55} & \ding{55}     & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               & \ding{55}                      & \checkmark                   \\
InstructDIAL           & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \checkmark & \checkmark  & \ding{55}                      & \ding{55} & \ding{55}     & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               &\checkmark                      & \ding{55}                    \\
Any-TOD                & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55}  & \checkmark & \ding{55}   & \ding{55}                      & \checkmark & \checkmark   & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               & \ding{55}                      & \checkmark                   \\
Vojita                 & \ding{55}  & \checkmark & \checkmark & \ding{55}  & \ding{55}  & \checkmark & \checkmark  & \checkmark                     & \ding{55} & \ding{55}     & \ding{55}  & \ding{55}  & \checkmark      & \checkmark   & \ding{55}     & \ding{55}               & \ding{55}                      & \checkmark                   \\
SGP-TOD                & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \ding{55}  & \ding{55}   & \ding{55}                      & \checkmark & \checkmark   & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               & \ding{55}                      & \checkmark                   \\
LDST                   & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \checkmark & \ding{55}   & \ding{55}                      & \ding{55} & \ding{55}     & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               &\checkmark                      & \ding{55}                    \\
Prompter               & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \checkmark & \ding{55}   & \ding{55}                      & \ding{55} & \ding{55}     & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               &\checkmark                      & \ding{55}                    \\
LUAS                   & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \ding{55}  & \checkmark & \checkmark  & \ding{55}                      & \ding{55} & \ding{55}     & \ding{55}  & \ding{55}  & \ding{55}       & \ding{55}    & \ding{55}     & \ding{55}               &\checkmark                      & \ding{55}                    \\
AutoTOD                & \checkmark & \checkmark & \ding{55}  & \checkmark & \ding{55}  & \ding{55}  & \ding{55}   & \ding{55}                      & \ding{55} & \ding{55}     & \checkmark & \checkmark & \checkmark      & \checkmark   & \ding{55}     & \ding{55}               & \ding{55}                      & \checkmark                   \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Comparison of TOD Models: Methods, Metrics, and Evaluation Approaches.} This table presents a comprehensive comparison of various Task-Oriented Dialogue (TOD) models, focusing on their evaluation metrics, tasks, and methods. It compares models across End-to-End (E2E) dialogue, Dialogue State Tracking (DST), Domain Detection, and Next-Action-Prediction (NAP) tasks, as well as human evaluation metrics such as Coherency, Fluency, Informativeness, Satisfaction, Understanding, and Truthfulness. The evaluation metrics include Inform (measuring if required information is provided), Success (task completion rate), BLEU (similarity between generated and reference responses based on n-grams), C (combined score, (Inform + Success) × 0.5 + BLEU), BERTScore (similarity using contextual embeddings), JGA (Joint Goal Accuracy), Slot-F1 (F1 score for slot-filling), Accuracy (general prediction correctness), and F1 (harmonic mean of precision and recall). The table also distinguishes between models using additional task-specific training (fine-tuning) and in-context learning (ICL, prompting). Models are marked with checkmarks ($\checkmark$) where evaluations were conducted, and crosses ($\times$) where not. This comparison underscores the need for consistent evaluation practices and transparency in code sharing to ensure reproducibility and fairness in TOD model assessments.}
\label{tab:my-table}
\end{table*}

==> tables/jga.tex <==
\begin{table*}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l c c c c c c c}
\toprule
\textbf{Model} & Attraction & Hotel & Restaurant & Taxi & Train & JGA (Average) \\ \midrule
\rowcolor{Gray}
\multicolumn{7}{c}{\textit{\textbf{\small MultiWOZ $\rightarrow$ MultiWOZ }}} \\
Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & --    \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --    \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --    \\ \midrule

\rowcolor{Gray}
\multicolumn{7}{c}{\textit{\textbf{\small MultiWOZ-SGD-Atis-Snips-Slurp $\rightarrow$ MultiWOZ }}} \\
Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & --    \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --    \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --    \\ \midrule

\rowcolor{Gray}
\multicolumn{7}{c}{\textit{\textbf{\small SGD-Atis-Snips-Slurp $\rightarrow$ MultiWOZ }}} \\
Llama 3.1 8B Instruct   & --    & --    & --    & --    & --    & --    \\
Llama 3.1 70B Instruct  & --    & --    & --    & --    & --    & --    \\
Llama 3.1 405B Instruct & --    & --    & --    & --    & --    & --    \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Performance comparison on different splits}.}
\label{tab:dst_result}
\vspace{-4.75mm}
\end{table*}

